Demand-Driven Pointer Analysis with Strong Updates via Value-Flow Refinement

We present a new demand-driven flow- and context-sensitive pointer analysis with strong updates for C programs, called SUPA, that enables computing points-to information via value-flow refinement, in environments with small time and memory budgets such as IDEs. We formulate SUPA by solving a graph reachability problem on an inter-procedural value-flow graph representing a program's def-use chains, which are pre-computed efficiently but over-approximately. To answer a client query (a request for a variable's points-to set), SUPA reasons about the flow of values along the pre-computed def-use chains sparsely (rather than across all program points), by performing only the work necessary for the query (rather than analyzing the whole program). In particular, strong updates are performed to filter out spurious def-use chains through value-flow refinement as long as the total budget is not exhausted. SUPA facilitates efficiency and precision tradeoffs by applying different pointer analyses in a hybrid multi-stage analysis framework. We have implemented SUPA in LLVM (3.5.0) and evaluate it by choosing uninitialized pointer detection as a major client on 18 open-source C programs. As the analysis budget increases, SUPA achieves improved precision, with its single-stage flow-sensitive analysis reaching 97.4% of that achieved by whole-program flow-sensitive analysis by consuming about 0.18 seconds and 65KB of memory per query, on average (with a budget of at most 10000 value-flow edges per query). With context-sensitivity also considered, SUPA's two- stage analysis becomes more precise for some programs but also incurs more analysis times. SUPA is also amenable to parallelization. A parallel implementation of its single-stage flow-sensitive analysis achieves a speedup of up to 6.9x with an average of 3.05x a 8-core machine with respect its sequential version.

==> intra_ex.tex <==
% !TEX root =  oopsla15.tex

\begin{figure*}[htbp]
	\begin{tabular}{l}
	\scalebox{0.92}{
		
%	\begin{tabular}{c}
%		\scalebox{0.8}{Auxiliary }\\
%		\scalebox{0.8}{Points-to} \\
%		\hline
%		\begin{tabular}{c}
%		$p\rightarrow m$ \\
%		$p\rightarrow n$ \\
%		$q\rightarrow m $
%		\end{tabular}
%		\\ \\ \\ \\ \\ \\ \\
%	\end{tabular}	
%	\quad


\begin{tabular}{l}
	\begin{tikzpicture}[thick]
	\begin{scope}[node distance=7.8mm]
	\node [](B_{1}) []{
	\begin{tabular}{c}
	\emph{*p=r}
	\end{tabular}
	};		   	
	\node [](B_{2}) [below=of B_{1}] {
	\begin{tabular}{c}
	\emph{v=*p}
	\end{tabular}
	};
	\node [](B_{3})  at ($(B_{2}) + (0.90, -1.25)$) {	
	\begin{tabular}{c}
	\emph{*q=s}
	\end{tabular}
	};				   				   
	\node [node distance=16.5mm](B_{4}) [below=of B_{2}] {	
	\begin{tabular}{c}
	\emph{*p=t} 
	\end{tabular}
	};

\scalebox{0.93}{
	\node [](L_{1})  at ($(B_{1}) + (-0.68, 0)$) {	
	$\lab_1\hspace{-1.2mm}:$
	};
	\node [](L_{2})  at ($(B_{2}) + (-0.68, -0.12)$) {	
	$\lab_2\hspace{-1.2mm}:$
	};
	\node [](L_{3})  at ($(B_{3}) + (-0.48, -0.23)$) {	
	$\lab_3\hspace{-1.2mm}:$
	};
	\node [](L_{4})  at ($(B_{4}) + (-0.65, -0.35)$) {	
	$\lab_4\hspace{-1.2mm}:$
	};
	\node [](L_{5})  at ($(B_{1}) + (-0.15, -0.15)$) {	
	$$
	};
	\node [](L_{6})  at ($(B_{2}) + (-1.6, -0.2)$) {	
	$$
	};
	\node [](L_{66})  at ($(B_{2}) + (-2.4, -0.2)$) {	
	$$
	};
	\node [](L_{7})  at ($(B_{1}) + (0.35, -0.15)$) {	
	$$
	};
	\node [](L_{8})  at ($(B_{2}) + (1.2, 0.30)$) {	
	$$
	};
	\node [](L_{9})  at ($(L_{6}) + (-0.05, 0)$) {	
	$[n]$
	};
	\node [](L_{99})  at ($(L_{6}) + (-0.8, 0)$) {	
	$[m]$
	};
	\node [](L_{10})  at ($(B_{1}) + (-0.5, -0.90)$) {	
	$[m]$
	};
	\node [](L_{110})  at ($(B_{1}) + (0.5, -0.90)$) {	
	$[n]$
	};
	\node [](L_{11})  at ($(L_{8}) + (0.3, 0.0)$) {	
	$[m]$
	};
	\node [](L_{12})  at ($(B_{3}) + (0.1, -0.90)$) {	
	$[m]$
	};
	\node [](L_{13})  at ($(B_{4}) + (0.0, -1.0)$) {	
		\hspace*{-4ex}$(a)$ Indirect def-use chains
	};
	\node [](L_{14})  at ($(B_{2}) + (-0.15, 0.1)$) {	
	};
	\node [](L_{15})  at ($(B_{2}) + (0.2, 0.1)$) {	
	};
	}								


	\path [densely dashed,->, thick, gray]    (B_{1}) edge  (L_{14});
	\path [densely dashed,->, thick, gray]    (B_{1}) edge  (L_{15});
		
	\path [densely dashed,->, thick, gray]    (B_{3}) edge  (B_{4});

	\draw [densely dashed,->, thick, gray] (L_{5}) .. controls (L_{66}) .. (B_{4});

	\draw [densely dashed,->, thick, gray] (L_{5}) .. controls (L_{6}) .. (B_{4});
	\draw [densely dashed,->, thick, gray] (L_{7}) .. controls (L_{8}) .. ($(B_{3}) + (-0.08,0.3)$);
	
	
	\end{scope}
	\end{tikzpicture}
	\end{tabular}	




	\begin{tabular}{l}
	\begin{tikzpicture}[thick]
	\begin{scope}[node distance=7.8mm]
	\node [](B_{1}) []{
	\begin{tabular}{c}
	\emph{*p=r}
	\end{tabular}
	};		   	
	\node [](B_{2}) [below=of B_{1}] {
	\begin{tabular}{c}
	\emph{v=*p}
	\end{tabular}
	};
	\node [](B_{3})  at ($(B_{2}) + (0.90, -1.25)$) {	
	\begin{tabular}{c}
	\emph{*q=s}
	\end{tabular}
	};				   				   
	\node [node distance=16.5mm](B_{4}) [below=of B_{2}] {	
	\begin{tabular}{c}
	\emph{*p=t} 
	\end{tabular}
	};

\scalebox{0.93}{
	\node [](L_{1})  at ($(B_{1}) + (-0.68, 0)$) {	
	$\lab_1\hspace{-1.2mm}:$
	};
	\node [](L_{2})  at ($(B_{2}) + (-0.68, -0.12)$) {	
	$\lab_2\hspace{-1.2mm}:$
	};
	\node [](L_{3})  at ($(B_{3}) + (-0.48, -0.23)$) {	
	$\lab_3\hspace{-1.2mm}:$
	};
	\node [](L_{4})  at ($(B_{4}) + (-0.65, -0.35)$) {	
	$\lab_4\hspace{-1.2mm}:$
	};
	\node [](L_{5})  at ($(B_{1}) + (-0.15, -0.15)$) {	
	$$
	};
	\node [](L_{6})  at ($(B_{2}) + (-1.6, -0.2)$) {	
	$$
	};
	\node [](L_{66})  at ($(B_{2}) + (-2.4, -0.2)$) {	
	$$
	};
	\node [](L_{7})  at ($(B_{1}) + (0.35, -0.15)$) {	
	$$
	};
	\node [](L_{8})  at ($(B_{2}) + (1.2, 0.30)$) {	
	$$
	};
	\node [](L_{9})  at ($(L_{6}) + (-0.05, 0)$) {	
	$[n]$
	};
	\node [](L_{99})  at ($(L_{6}) + (-0.8, 0)$) {	
	$[m]$
	};
	\node [](L_{10})  at ($(B_{1}) + (-0.5, -0.90)$) {	
	$[m]$
	};
	\node [](L_{110})  at ($(B_{1}) + (0.5, -0.90)$) {	
	$[n]$
	};
	\node [](L_{11})  at ($(L_{8}) + (0.3, 0.0)$) {	
	$[m]$
	};
	\node [](L_{12})  at ($(B_{3}) + (0.1, -0.90)$) {	
	$[m]$
	};
	\node [](L_{13})  at ($(B_{4}) + (0.0, -1.0)$) {	
		\hspace*{-4ex}$(a)$ Indirect def-use chains
	};
	\node [](L_{14})  at ($(B_{2}) + (-0.15, 0.1)$) {	
	};
	\node [](L_{15})  at ($(B_{2}) + (0.2, 0.1)$) {	
	};
	}								


	\path [densely dashed,->, thick, gray]    (B_{1}) edge  (L_{14});
	\path [densely dashed,->, thick, gray]    (B_{1}) edge  (L_{15});
		
	\path [densely dashed,->, thick, gray]    (B_{3}) edge  (B_{4});

	\draw [densely dashed,->, thick, gray] (L_{5}) .. controls (L_{66}) .. (B_{4});

	\draw [densely dashed,->, thick, gray] (L_{5}) .. controls (L_{6}) .. (B_{4});
	\draw [densely dashed,->, thick, gray] (L_{7}) .. controls (L_{8}) .. ($(B_{3}) + (-0.08,0.3)$);
	
	
	\end{scope}
	\end{tikzpicture}
	\end{tabular}	
	}
	\end{tabular}
	\caption{An intra-procedural example}
\end{figure*}
	
	
	
	

==> table.tex <==
\clearpage

\section{Program Statistics}
\label{sec:tab}



\begin{table}[!htbp]
\begin{center}
\scalebox{0.8}{
\hspace{-2mm}
\setlength{\tabcolsep}{4.8pt}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}\hline \hline 

  \multicolumn{1}{|c|}{\multirow{2}{*}{Program}} & \multicolumn{1}{c|}{\multirow{2}{*}{KLOC}} & \multicolumn{5}{c|}{Statements} & \multicolumn{1}{c|}{Top-Level} & \multicolumn{5}{c|}{Address-Taken Objects} & \multicolumn{2}{c|}{Call Sites} & \multicolumn{1}{c|}{\multirow{2}{*}{Queries}} \\ \cline{3-7} \cline{9-15}

   & & \multicolumn{1}{c|}{Addr} & \multicolumn{1}{c|}{Copy} & \multicolumn{1}{c|}{Phi} & \multicolumn{1}{c|}{Load} & \multicolumn{1}{c|}{Store} & \multicolumn{1}{c|}{Pointers} & \multicolumn{1}{c|}{Global} & \multicolumn{1}{c|}{Heap} & \multicolumn{1}{c|}{Stack} & \multicolumn{1}{c|}{Func} & \multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{Direct} & \multicolumn{1}{c|}{Indirect} & \\ \hline \hline

milc-v6 & 15.0 & 1275 & 8297 & 537 & 1138 & 466 & 29584 & 92 & 63 & 203 & 272 & 865 & 26062 & 4 & 3 \\ \hline
less-451 & 27.1 & 1660 & 2316 & 874 & 1060 & 856 & 22835 & 305 & 37 & 133 & 507 & 1135 & 16306 & 5 & 100 \\ \hline
hmmer-2.3 & 36.0 & 2447 & 16578 & 1607 & 6224 & 1068 & 74689 & 76 & 164 & 274 & 602 & 1472 & 61925 & 9 & 2043 \\ \hline
make-4.1 & 40.4 & 2559 & 5479 & 3040 & 2344 & 1504 & 36707 & 181 & 45 & 255 & 426 & 1563 & 37903 & 9 & 1133 \\ \hline
a2ps-4.14 & 64.6 & 6326 & 24049 & 5122 & 10337 & 3338 & 116129 & 283 & 260 & 308 & 1798 & 3625 & 111336 & 99 & 5065 \\ \hline
bison-3.0.4 & 113.3 & 3304 & 17282 & 4135 & 8363 & 3731 & 90049 & 295 & 103 & 227 & 797 & 1976 & 86625 & 293 & 4408 \\ \hline
grep-2.21 & 118.4 & 1423 & 4647 & 1566 & 1540 & 1023 & 33931 & 128 & 51 & 157 & 385 & 1108 & 23800 & 45 & 562 \\ \hline
tar-1.28 & 132.0 & 5044 & 12625 & 4567 & 4907 & 3361 & 85727 & 348 & 161 & 449 & 1011 & 3350 & 72184 & 465 & 909 \\ \hline
bash-4.3 & 155.9 & 8946 & 26186 & 8479 & 10456 & 5375 & 191413 & 1066 & 69 & 875 & 2681 & 6359 & 146771 & 126 & 5103 \\ \hline
sendmail-8.15.1 & 259.9 & 13416 & 38809 & 11362 & 12860 & 10206 & 256074 & 856 & 173 & 1456 & 2335 & 7549 & 227441 & 411 & 2715 \\ \hline
vim-7.4 & 413.1 & 15365 & 66500 & 20159 & 27764 & 17762 & 466493 & 1581 & 183 & 1912 & 3206 & 8960 & 369359 & 1555 & 6753 \\ \hline
emacs-24.4 & 431.9 & 17149 & 107539 & 11628 & 29712 & 23069 & 754746 & 3445 & 268 & 2089 & 3938 & 12037 & 431891 & 447 & 4438 \\ \hline

\end{tabular}
}
\caption{Program characteristics
\label{tab:stat}}
\end{center}
\end{table}

\clearpage

